Language Chameleon: Transformation analysis between languages using Cross-lingual Post-training based on Pre-trained language models

As pre-trained language models become more resource-demanding, the inequality between resource-rich languages such as English and resource-scarce languages is worsening. This can be attributed to the fact that the amount of available training data in each language follows the power-law distribution, and most of the languages belong to the long tail of the distribution. Some research areas attempt to mitigate this problem. For example, in cross-lingual transfer learning and multilingual training, the goal is to benefit long-tail languages via the knowledge acquired from resource-rich languages. Although being successful, existing work has mainly focused on experimenting on as many languages as possible. As a result, targeted in-depth analysis is mostly absent. In this study, we focus on a single low-resource language and perform extensive evaluation and probing experiments using cross-lingual post-training (XPT). To make the transfer scenario challenging, we choose Korean as the target language, as it is a language isolate and thus shares almost no typology with English. Results show that XPT not only outperforms or performs on par with monolingual models trained with orders of magnitudes more data but also is highly efficient in the transfer process.

==> backup.tex <==
\section{Multilingual PLM의 비교}
multilingual pre-trained language model은 여러언어의 공통 언어적 자질을 학습함으로서 여러언어를 하나의 구조로 극복할 가능성을 보여준다. 단일 저자원 언어 모델을 처음부터 학습하는 것은 언어 데이터의 양 문제로 처음부터 학습하는 것에 문제가 있지만, 다국어 사전학습모델을 사용하면 고자원 언어를 이용하여 데이터 리소스 문제를 어느 정도 해결할 수 있다. 이 섹션에서는 cross-lingual post-training을 진행한 모델과 한국어를 포함하는 다국어 사전학습 모델을 architecture로 나누어 설명한다.

\paragraph{Encoder Structure}
인코더 계층으로만 구성된 다국어 사전학습 모델은 저자원 언어의 Natural Language Understanding 태스크 성능을 높이기 위한 연구가 이루어지고 있다. BERT와 동일한 방법으로 학습된 mBERT 및 distil-mBERT, BERT 계열과 동일하게 MLM을 pre-training task로 하는 Cross-lingual Language Model Pre-training(xlm)및 XLM과 그 variant인 XLM-E, XLM-align이 등장하였다. 또한 multilingual LUKE(mLUKE)은 MLM과 함께 Masked Entity Prediction (MEP)로 학습되었으며, infoXLM은 MLM, 병렬 데이터셋의 소스 문장과 타겟 문장을 연결하여 임베딩을 구성하는 Translation Language Modeling (TLM), 소스 언어와 타겟 언어의 시퀀스 정보의 유사도를 최대화 하는 Cross-lingual Contrastive Learning (XlCO)를 pre-training task로 하는 infoXLM도 등장하였다. 
AMBER는 MLM, TLM, WA, SA로 학습되었으며, Unicoder는 MLM, TLM뿐만 아니라, 병렬 문장 사이의 단어 정렬을 학습하도록 하는 Cross-lingual Word Recovery (ClWR), 소스 문장과 타겟 문장의 이미가 동일한지 분류하여 문장 사이의 cross-linguality를 하는 Cross-lingual Paraphrase Classification (CIPC), 다국어 문서에서의 MLM을 수행하여 document-level의 perplexity를 낮추는 Cross-lingual Masked Language Modeling (CIMLM)을 활용한다. 

\paragraph{Decoder Structure}
디코더 계층만으로 이루어진 다국어 모델은 GPT3와 같이 아주 많은 파라미터 수를 가지는 빅모델이다. GPT-3는 대량의 코퍼스에서 포함된 여러 언어로 딕셔너리를 구성하여 학습하였고, 대략 120개의 언어를 포함한다. 또한, GPT-3는 GPT-2와 같이 별도의 cross-linguality 표현을 학습하는 사전학습 방법 없이 단순히 Casual Language Modeling (CLM)만으로 cross-linguality를 높였다. 


\paragraph{Encoder-Decoder Structure}
Natural Language Generation 태스크를 수행하고자 인코더-디코더 계층을 모두 가진 다국어 사전학습 모델이 있다. 대표적으로 mBART 및 MASS 모델은 다중 언어 문장에 손상을 준 후 원본 문장을 복원하는 Multilingual Denoising Pretraining (MDP)을 적용하여 다중 언어에 대한 표현력을 학습하였다. XNLG는 mBART와 유사하게 Denoising Auto-Encoding (DAE), Cross-lingual MLM (XMLM), 소스 문장과 동일한 언어의 문장을 생성하는 DAE 방식의 Cross-Lingual Auto-Encoding (XAE) 사전학습 접근법을 제안했다. XNLG 모델은 MLM과 DAE 사전학습 태스크를 해결하면서 단일 언어 표현력 (monolingual representation)을 확장하면서, XMLM과 XAE 사전학습 태스크를 통해 다중언어의 cross-lingual 표현력을 확장하여 언어간의 다양한 자연어 생성 태스크의 성능을 높였다. 또한, 모델의 크기를 기하급수적으로 키우고, MLM-SC를 pre-training task로 하는 mT5와, 다중언어에 대한 MLM (CS-MLM)를 통해 Cross-lingual generation 태스크에 대한 성능을 높인 VECO, 병렬 쌍의 문장에 대해 마스킹된 span을 예측하는 Translation Pair Span-Corruption (TPSC), 단일언어의 문장에 대해 마스킹된 span을 예측하는 Translation Span-Corruption (TSC)가 등장하였다.

\section{Korean PLM의 비교}
English PLM의 발전과 더불어, 다양한 Korean Pre-trained language model이 제안되었다. 다양한 기업, 개인, 학계에서 Transformer의 encoder, decoder를 기반으로 하는 모델을 공개하였다. 이 section에서는 encoder, decoder, encoder-decoder 구조로 나누어 해당 모델들을 설명한다. 

\paragraph{Encoder Structure}
BERT와 동일한 구조 및 pre-training task인 MLM, NSP를 사용하여 만들어진 KoBERT를 시작으로, KorBERT, HanBERT, KLUE-BERT, KRBERT등 다양한 Korean BERT model이 등장하였다. SentencePiece, WordPiece 등 모델마다 다양한 tokenizer가 사용되었으며, 다양한 종류와 분량의 한국어 corpus 데이터로 학습되었다. 특히 KLUE-BERT는 KLUE-BERT는 한국어 벤치마크 데이터인 KLUE에서 베이스라인으로 사용되었던 모델이다. 또한 BERT모델을 경량화한 distilBERT나 ALBERT를 오마주한 distilKoBERT, KALBERT, KB-ALBERT도 등장하였으며, 한국어 버전의 ALBERT인 albert-kor-base model도 공개되었다. ELECTRA를 본따 Replaced Token Detection task(RTD)를 pre-training task로 하는 KoELECTRA와, BigBird model와 마찬가지로 일반적인 BERT보다 더 긴 sequence 다룰 수 있는 KoBigBird가 등장했다. 
또한 wikipedia, newspaper, 청원문서와 같은 formal corpus 뿐만 아니라, Korean Comment 데이터로 학습되어 colloquial한 특성이 더 반영된 KcBERT, KcELECTRA도 제안되었다.

\paragraph{Decoder Structure}
한국어 버전의 GPT2 모델인 KoGPT2는 GPT2와 마찬가지로 transformer decoder 구조를 가지고 있으며, Next Token Prediction(NTP)을 통해 사전학습되었다. 또한 KoGPT-Trinity는 KoGPT2보다 훨씬 큰 파라미터 개수를 가진 모델이다. KoGPT3의 구조를 모방한 KoGPT와, 최대 82.0B의 크기를 가진 초거대모델 HyperCLOVA도 공개되었다. 

\paragraph{Encoder-Decoder Structure}
encoder-decoder 구조의 대표적인 모델은 BART, Text-to-Text Transfer Transformer(T5)이다. Next token prediction(NTP)을 통해 사전학습되었으며 BART와 동일한 구조를 가진, 즉 한국어 버전의 BART 모델인 KoBART가 공개되었다. 또한 한국어와 영어 버전의 T5를 모방한 KE-T5와, T5에서의 mask-fill과 GPT3에서의 Next Token Prediction을 동시에 사전학습한 ET-5도 공개되었다. 


==> table/result2+3.tex <==
\begin{table*}[ht]

\centering
\renewcommand{\arraystretch}{1.4}

\begin{subtable}{1\textwidth}
\scalebox{0.63}{
\begin{tabular}{l||c|cc|c|cc|cc|cccc|cc}
\hline
            & YNAT                          & \multicolumn{2}{c|}{KLUE-STS}                                                               & KLUE-NLI                               & \multicolumn{2}{c|}{KLUE-NER}                                                      & \multicolumn{2}{c|}{KLUE-RE}                                                                  & \multicolumn{4}{c|}{KLUE-DP}                                                                                                                                                                      & \multicolumn{2}{c}{KLUE-MRC}                                                                                                          \\ \cline{2-15} 
            & F1                            & \multicolumn{1}{c}{R^P}                   & F1                            & ACC                                    & \multicolumn{1}{c}{F1^E}         & F1^C         & \multicolumn{1}{c}{F1^{mic}}         & AUC                           & \multicolumn{1}{c}{UAS^{mac}}  & \multicolumn{1}{c}{UAS^{mic}}  & \multicolumn{1}{c}{LAS^{mac}}  & LAS^{mic}  & \multicolumn{1}{c}{EM}                                                   & ROUGE                                                \\ \hline \hline
\begin{tabular}[c]{@{}c@{}}KoELECTRA-400K\end{tabular}  & 4.17  & \multicolumn{1}{c}{7.79}             & 0.00          & 33.33    & \multicolumn{1}{c}{0.00}              & 6.77                 & \multicolumn{1}{c}{0.00}     & 3.47  & \multicolumn{1}{c}{83.14}          & \multicolumn{1}{c}{85.82}          & \multicolumn{1}{c}{78.73}          & 81.70          & \multicolumn{1}{c}{5.08}         & 7.87  \\ 
\begin{tabular}[c]{@{}c@{}}KoELECTRA-4M\end{tabular} & 2.40  & \multicolumn{1}{c}{10.21}            & 0.00          & 33.33    & \multicolumn{1}{c}{0.00}              & 6.77                 & \multicolumn{1}{c}{0.00}     & 3.15  & \multicolumn{1}{c}{68.52}          & \multicolumn{1}{c}{71.99}          & \multicolumn{1}{c}{55.62}          & 65.75          & \multicolumn{1}{c}{0.00}         & 3.69  \\ \hline
\begin{tabular}[c]{@{}c@{}}XPT-400K\end{tabular}        & 83.23 & \multicolumn{1}{c}{76.67}            & 75.55         & 64.03    & \multicolumn{1}{c}{66.95}             & 88.53                & \multicolumn{1}{c}{54.63}    & 52.08 & \multicolumn{1}{c}{91.06}          & \multicolumn{1}{c}{92.24}          & \multicolumn{1}{c}{85.71}          & 89.93          & \multicolumn{1}{c}{26.07}        & 48.73 \\ 
\begin{tabular}[c]{@{}c@{}}XPT-4M\end{tabular}       & \textbf{86.53} & \multicolumn{1}{c}{\textbf{84.23}}            & \textbf{90.30}          & \textbf{82.03}    & \multicolumn{1}{c}{\textbf{70.42}}             & \textbf{91.24}                & \multicolumn{1}{c}{\textbf{67.31}}    & \textbf{72.56} & \multicolumn{1}{c}{\textbf{93.78}}          & \multicolumn{1}{c}{\textbf{94.61}}          & \multicolumn{1}{c}{\textbf{87.54}}          & \textbf{92.69}          & \multicolumn{1}{c}{\textbf{30.39}}        & \textbf{59.18}  \\ \hline 
\end{tabular}
}
\caption{400K, 4M한국어 코퍼스로 pretraining한 한국어 언어모델 KoELECTRA-400K, KoELECTRA-4M 동일한 코퍼스로 XPT를 적용한 XPT-400K, XPT-4M 모델의 Klue dataset에 대한 성능 평가 결과 표. }
\label{tab:result_KoELEC2}
\end{subtable}

\bigskip
\begin{subtable}{1\textwidth}
\scalebox{0.63}{
\begin{tabular}{l||c|cc|c|cc|cc|cccc|cc}
\hline
            & YNAT                          & \multicolumn{2}{c|}{KLUE-STS}                                                               & KLUE-NLI                               & \multicolumn{2}{c|}{KLUE-NER}                                                      & \multicolumn{2}{c|}{KLUE-RE}                                                                  & \multicolumn{4}{c|}{KLUE-DP}                                                                                                                                                                      & \multicolumn{2}{c}{KLUE-MRC}                                                                                                          \\ \cline{2-15} 
            & F1                            & \multicolumn{1}{c}{R^P}                   & F1                            & ACC                                    & \multicolumn{1}{c}{F1^E}         & F1^C         & \multicolumn{1}{c}{F1^{mic}}         & AUC                           & \multicolumn{1}{c}{UAS^{mac}}  & \multicolumn{1}{c}{UAS^{mic}}  & \multicolumn{1}{c}{LAS^{mac}}  & LAS^{mic}  & \multicolumn{1}{c}{EM}                                                   & ROUGE                                                \\ \hline \hline
\begin{tabular}[c]{@{}l@{}}XPT-4M\\ with RoBERTa-random \end{tabular} & 85.67     & 77.52    & 75.35                       & 69.63        & 69.28                 & 90.12                   & 47.24           & 44.99   & 92.76              & 93.89             & 86.38           & 91.70      & 24.82       & 47.39  \\ \hline
XPT-4M                                                                              & \textbf{86.53} & \textbf{84.23}                       & \textbf{90.30}                  & \textbf{82.03}   & \textbf{70.42}             & \textbf{91.24}                & \textbf{67.31}        & \textbf{72.56}    & \textbf{93.78}          & \textbf{94.61}          & \textbf{87.54}          & \textbf{92.69}          & \textbf{30.39}          & \textbf{59.18} \\ \hline
\end{tabular}
}
\caption{source language $\protect L_T$의 사전학습언어모델인 RoBERTa의 파라미터를 random initlize한 뒤 4M의 target language $\protect L_S$ 의 코퍼스로 scratch부터 학습한 모델과 XPT 모델을 비교한 표. }
\label{tab:result_random2}
\end{subtable}

\caption{4M의 데이터로 학습한 XPT와 다른 모델을 비교한 결과. $\protect R^{P}$와 $\protect R^{S}$ 는 Pearson’s $\protect \textit{r}$ 과 Spearman $\protect \textit{r}$를 의미한다. $\protect F1^{E}$,$\protect F1^{C}$ 그리고 $\protect F1^{mic}$는 각각 entity\char`_micro\char`_F1, character\char`_micro\char`_F1 그리고 micro\char`_F1를 의미한다. $\protect UAS^{mac}$, $\protect UAS^{mic}$, $\protect LAS^{mac}$ 그리고 $\protect LAS^{mic}$는 각각 uas\char`_macro\char`_f1, uas\char`_micro\char`_f1, las\char`_macro\char`_f1 그리고 las\char`_micro\char`_f1를 말한다. Best performances are highlighted in bold.}
\label{tab:result2+3}
\end{table*}
